Carrot and Stick: Eliciting Comparison Data and Beyond

Comparison data elicited from people are fundamental to many machine learning tasks, including reinforcement learning from human feedback for large language models and estimating ranking models. They are typically subjective and not directly verifiable. How to truthfully elicit such comparison data from rational individuals? We design peer prediction mechanisms for eliciting comparison data using a bonus-penalty payment. Our design leverages on the strong stochastic transitivity for comparison data to create symmetrically strongly truthful mechanisms such that truth-telling 1) forms a strict Bayesian Nash equilibrium, and 2) yields the highest payment among all symmetric equilibria. Each individual only needs to evaluate one pair of items and report her comparison in our mechanism. We further extend the bonus-penalty payment concept to eliciting networked data, designing a symmetrically strongly truthful mechanism when agents' private signals are sampled according to the Ising models. We provide the necessary and sufficient conditions for our bonus-penalty payment to have truth-telling as a strict Bayesian Nash equilibrium. Experiments on two real-world datasets further support our theoretical discoveries.

==> sections/model-old.tex <==


\section{Background and problem formulation}\label{sec:model}
scalar $s$, random variable $\rs$, vector $\vs$, random vector $\rvs$.\fang{$i$ for Isabel, $j$ for Julia, and $k$ for Ken?}

\fang{we start with comparison data and will generalize to }
\subsection{Peer prediction mechanism}
Given a collection of items $\mathcal{A}$ and a set of strategic agents $\mathcal{N}$, we want to collect noisy comparison between pairs of items from those strategic agents.\fang{ for downstream learning tasks?}  To incentivize agent's truthful reports, a peer prediction mechanism creates a game between those strategic agents outlined below:\fang{should we remove enumerate environment?}
\begin{enumerate}
    \item We first choose an \emph{assignment matrix} $\mathcal{E} = \{e_i = (a_{u_i}, a_{v_i}): i\in \mathcal{N}\}$  where agent $i\in \mathcal{N}$ gets a pair of items $e_i = (a_{u_i}, a_{v_i})\in \mathcal{A}^2$ to compare.\fang{More formally $\mathcal{E} = \{(i, e_i)\}$ which include pairs of items as well as the who work on which pair.}  
    \item Each agent $i\in \mathcal{N}$ privately observes the realization of the comparison (signal) $s_i\in \{-1, 1\}$ where $1$ represent item $a_{u_i}$ is preferred over item $a_{v_i}$, and reports $\hat{s}_i\in \{-1, 1\}$ potentially different from her signal.  Let ${\vs} = (s_i)_{i\in \mathcal{N}}$ be all agents' private signals and $\hat{\vs} = (\hat{s}_i)_{i\in \mathcal{N}}$ be all agents' reports.  All agents' signal are jointly generated from a random vector $\rvs = (\rs_i)_{i\in \mathcal{N}}$ with a probability measure $P$ called the common prior so that $\vs \sim \rvs$.  We will specify our common prior for comparison data in \cref{sec:sstmodel}. 
    \item Finally, we run a \emph{peer prediction mechanism} $(M_i)_{i\in \mathcal{N}}$ which takes all agents' reports $\hat{\vs}$ and pays agent $i$ with $M_i(\hat{\vs})\in \R$.   \fang{one agent multiple tasks?}
\end{enumerate}




Each agent $i$'s strategy is a random function from her signal to a report $\sigma_i: s_i\mapsto \hat{s}_i$, and the randomness of their strategies is independent of each other's.  With slight abuse of notation, we write $\sigma_i(s_i, \hat{s}_i) = \Pr[\hat{\rs}_i = \hat{s}_i\mid \rs_i = s_i]$ as the conditional probability of reporting $\hat{s}_i$ given private signal $s_i$.  A strategy profile $\bm{\sigma}$ is a collection of all agent's strategies.  All agents are rational and risk-neutral, so they want to maximize their expected payments.  Thus, given a common prior $P$ and a strategy profile $\bm{\sigma}$, agent $i$ wants to maximize her ex-ante payment denoted as $\E_{\bm{\sigma}, P}[M_i(\hat{\rvs})]$ where $\hat{\rvs}$ is the random vector of all agents' report that depends on the signals $\rvs$ and strategy profile $\bm{\sigma}$.   

% We want to design a peer prediction mechanism to elicit all agents to report their signals truthfully without verification.  
We introduce three families of strategies, truth-telling, permutation, and uninformed strategy profiles, which are central to understanding and designing effective peer prediction mechanisms.  
\begin{itemize}
    \item A strategy is \emph{truthful} (or truth-telling) if it is an identity map, meaning the agent reports her signal without any manipulation, and a strategy profile is truthful if all agents' strategies are truthful.  
    \item Another important family is \emph{permutation strategy profiles}, where agents simultaneously relabel their signals, which is indistinguishable from truth-telling unless the peer prediction mechanism has additional knowledge about the common prior.   
    \item Finally, a strategy is \emph{uninformed} if it has the same report distribution across all signals, and it is informed otherwise.  Common examples include consistently reporting all signals as a constant value, such as $1$ or $-1$, or using a random report regardless of the signal.   Uninformed strategies are undesirable as the reports bear no relationship to the private signals.   
\end{itemize}A strategy profile is \emph{symmetric} if all agents use the same strategy.  For example, both truth-telling and permutation strategy profiles are symmetric.

% \paragraph{Equilibria and Goals}
Now, we introduce goals for a peer prediction mechanism that favors truth-telling more than other strategies.  First, we want the truth-telling (strategy profile) to be a strict \emph{Bayesian Nash equilibrium} so that any agent's payment would strictly decrease if she unilaterally changes to any non-truthful strategy.  We will call Bayesian Nash equilibrium as equilibrium for short.  Moreover, there may be multiple equilibria, and a desirable mechanism should ensure that truth-telling is better than all other equilibria.  In this paper, we aim for symmetrically strongly truthful mechanisms defined below.
\begin{definition}
    A peer prediction mechanism is \defn{symmetrically strongly truthful} if the truth-telling is a strict equilibrium, and each agent's expected payment in truth-telling is no less than the payment in any other symmetric equilibria with equality for permutation strategy profiles.  
\end{definition}
Note that \cite{kong2016framework} shows that it is impossible to design mechanisms that pay the truth-telling strategy profile strictly better than other permutation strategy profiles without additional knowledge of the common prior.\yc{Explain earlier why permutation equilibrium has the same payoff as truthful equilibrium without any additional information. Cite some papers.}\fang{footnote?}

 





\subsection{Bayesian SST model for comparison data}\label{sec:sstmodel}
We introduce Bayesian SST models as the common priors for comparison data using the concept of \emph{strong stochastic transitivity} (\cref{def:transitive}), which is a well-founded property of comparison in social science and psychology (e.g., see \citet{fishburn1973binary} for an overview).  Given $\mathcal{A}$, the full set of all possible  comparisons described by \emph{comparison function} $t: \mathcal{A}\times \mathcal{A}\to \{-1,1\}$ where for any $a\neq a'$, $t(a,a') = \{-1,1\}$ and $t(a,a') = -t(a',a)$. Intuitively, a comparison function is strongly stochastically transitive if for any three items $a, a', a''$ if $a$ is more favorable than $a'$ and $a'$ is more favorable than $a''$, strong stochastic transitivity implies $a$ is even more favorable than $a''$. 
\begin{definition}[\cite{vail1953stochastic,davidson1959experimental}]\label{def:transitive}
    A stochastic comparison function on $\mathcal{A}$, $\rt:\mathcal{A}^2\to \{-1, 1\}$, is \fang{strict} \defn{strongly stochastically transitive} if for all $a, a', a''\in \mathcal{A}$ with $\Pr[\rt(a, a') = 1]> 1/2$ and $\Pr[\rt(a', a'') = 1]> 1/2$, then 
    $$\Pr[\rt(a, a'') = 1]> \max \{\Pr[\rt(a, a') = 1], \Pr[\rt(a', a'') = 1]\}.$$
\end{definition}



We consider a family of stochastic comparison functions $\rs$ called \defn{Bayesian SST model}\fang{better name?} where each $\rs$ consists of a family of strongly stochastically transitive comparison functions $(T_\theta)_{\theta\in \Theta}$ and a distribution on parameter $\mu_\theta$ where the parameter $\theta$ can be each item's score (\cref{ex:para}) or a reference ranking (\cref{ex:mallows}).   First $\theta$ is sampled from $\mu_\theta$, and the comparison between each pair $(a, a')$ $\rs(a, a')$ is independently sampled according to $T_\theta(a, a')$.  Under an Bayesian SST model, each agent $i\in \mathcal{N}$ has the knowledge of $(T_\theta)_{\theta\in \Theta}$ and $\mu_\theta$, and observe a comparison from the assigned pair $\rs_i = \rs(a_{u_i}, a_{v_i})$.  We assume items are a priori similar but ex-post distinct so that for all $a, a'\in \mathcal{A}$, $\E[\rs(a, a')] = \E[\E[\rt_\theta(a, a')\mid \theta]] = 0$ and $\E[\rt_\theta(a,a')\mid \theta]\neq 0$ for all $\theta$.  
Below we show that several classical models including Bradley-Terry Luce~\cite{bradley1952rank,luce2005individual}, Thurstone (Case V)~\cite{thurstone2017law}, and Mallows $\eta$-model~\cite{1379e110-3390-3287-8a9b-6ccafc65156a} are special cases of our Bayesian SST model. 
\yc{What is $\theta$?}\yc{Is Plackett-Luce also a special case of this model?}\fang{I am not sure what is the difference.  It seems like Plackett-Luce with score function $score$ has $\Pr[ T_\theta(a, a) = 1] = \frac{score(a)}{score(a)+score(a')}$.  If we can define $score (a) = \exp(\theta_a)$, the model reduce to Bradley-Terry with $\theta_a$}


\begin{example}[Bradley-Terry-Luce, Thurstone model, and more~\cite{tversky1969substitutability}]\label{ex:para}
Let $\theta\in \R^\mathcal{A} = \Theta$ where each coordinate are independently and identically sampled from a fixed non-atomic distribution $\nu$ on $\R$ \fang{continues distribution to avoid $\theta_a = \theta_{a'}$.  Exchangeable is sufficient}, and each item $a$ have a scalar quality $\theta_a\in \mathbb{R}$.  Let $F:
\R\to [0,1]$ be any strictly increasing function  such that $F(t) = 1-F(-t)$ for all $t\in \R$. Conditional a fixed $\theta$, 
$$\Pr[T_\theta(a, a') = 1] = F\left(\theta_a-\theta_{a'}\right)\text{ for all }a, a'\in \mathcal{A}.$$
This model recovers the Thurstone model~\cite{thurstone2017law} by setting $F(t) = \Phi(t)$ where $\Phi$ is the Gaussian CDF, and the Bradley-Terry-Luce model~\cite{bradley1952rank} by setting $F(t) = \frac{e^t}{1+e^t}$, the sigmoid function.  Moreover, this model also contains any additive random utility model~\cite{azari2012random} where $T(a,a') = 1$ if $\theta_a+\rz>\theta_{a'}+\rz'$ with iid noise $\rz$ and $\rz'$, because we can set $F$ to be the CDF of the difference of two iid noise. 
\end{example}

\begin{proposition}\label{prop:para}
    For any strictly increasing $F$ and non-atomic $\nu$ on $\R$, the parametric model in \cref{ex:para} is an Bayesian SST model.
\end{proposition}
The proof is similar to proving the parameter model is strongly stochastically transitive~\cite{shah2016stochastically}, but is included in appendix for completeness.

\begin{example}[Mallows $\eta$-model~\cite{1379e110-3390-3287-8a9b-6ccafc65156a}]\label{ex:mallows} Let $\Theta$ be the set of rankings on $\mathcal{A}$ and $\eta>0$ be a dispersion parameter.  Given a reference ranking $\theta\in \Theta$, the \emph{Mallows $\eta$-model} generate a ranking $\phi\in \Theta$ with probability
$\Pr(\phi) \propto \exp(-\eta d(\theta, \phi))$
where $d(\theta, \phi)$ can be Kendall's tau distance, $\left|\{(a, a')\in \mathcal{A}^2: \theta(a)<\theta(a')\text{ and }\phi(a)>\phi(a')\}\right|$ and $\theta(a)$ is the rank of item $a$.  
Therefore, to generate comparisons, we first sample an uniform $\theta$ and 
\begin{equation*}
    \Pr[T_\theta(a, a') = 1] = \sum_{\phi: \phi(a)>\phi(a')}\Pr(\phi), \text{ for all }a, a'\in \mathcal{A}.
\end{equation*}

% \fang{Mallows model should have sst: mentioned in Section 6 of \citet{haddenhorst2020generalized}.  However, I cannot find a formal statement.  We may need to read the original paper~\cite{1379e110-3390-3287-8a9b-6ccafc65156a} section 9.}
\end{example}


\begin{proposition}\label{prop:mallows}
    For any $\eta>0$, Mallows $\eta$-model in \cref{ex:mallows} with uniform distribution on reference ranking is an Bayesian SST model.  
\end{proposition}
The proof is similar to proving Mallows model is strongly stochastically transitive (e.g., \cite{pmlr-v32-busa-fekete14}), but is included in appendix for completeness.

